Practical Modulo Sampling: Mitigating High-Frequency Components

Recovering signals within limited dynamic range (DR) constraints remains a central challenge for analog-to-digital converters (ADCs). To prevent data loss, an ADCs DR typically must exceed that of the input signal. Modulo sampling has recently gained attention as a promising approach for addressing DR limitations across various signal classes. However, existing methods often rely on ideal ADCs capable of capturing the high frequencies introduced by the modulo operator, which is impractical in real-world hardware applications. This paper introduces an innovative hardware-based sampling approach that addresses these high-frequency components using an analog mixer followed by a Low-Pass Filter (LPF). This allows the use of realistic ADCs, which do not need to handle frequencies beyond the intended sampling rate. Our method eliminates the requirement for high-specification ADCs and demonstrates that the resulting samples are equivalent to those from an ideal high-spec ADC. Consequently, any existing modulo recovery algorithm can be applied effectively. We present a practical hardware prototype of this approach, validated through both simulations and hardware recovery experiments. Using a recovery method designed to handle quantization noise, we show that our approach effectively manages high-frequency artifacts, enabling reliable modulo recovery with realistic ADCs. These findings confirm that our hardware solution not only outperforms conventional methods in high-precision settings but also demonstrates significant real-world applicability.

==> hardware_old.tex <==
\section{Realistic Modulo Hardware Prototype}
\label{sec:hardware}

\section{System Architecture}
	\label{sec: system architecture}
	In this section, we elaborate on the system architecture of the hardware prototype; there are four different analog input channels, and a 50KHz sampling device is used for each channel, all four ADCs are using the sampling clock generated by the  TEENSY-M. First, we present the high-level system architecture, after which we discuss the concrete structure of the hardware components.

\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth, height=6cm]{fig/System Architecture.png}
  \caption{Four different analog input signals with four synchronized 50KHz ADC samplers}
  \label{Fig: System Block Diagram}
\end{figure}

\subsection{High-Level Design}
	 Sampler 1 receive the input signal (Sia) from Channel 1, Sampler 2 receive the modulo signal generated by the UDR at Channel 2, Sampler 3 receive the modulo signal multiplied by 50KHz comb generator after 25KHz LPF at channel 3, and Sampler 4 samples the UDR modulo signal with 25KHz LPF at channel 4. The 50KHz clock that synchronize all four ADC's is generated by the TEENSY M at channel 3, whenever the input signal cross threshold level, the it is Folded to specific boundary at that time, and set a folded signal out for the two controllers TEENSY-M and TEENSY-S1, this  effect the LSB Bit for the next ADC's word sampled.
        


\begin{figure}[h]
  \centering
  \includegraphics[width=1\columnwidth, height=6cm]{fig/Multiply COMB Gen.png}
  \caption{Multiply Signal In with COMB Generator with 50KHz steps, the multiplied signal is then passed through a 25KHz Low pass filter, then to the ADC 50KHz sampler}
  \label{Fig: COMB Gen Block Diagram}
\end{figure}

\subsection{Multiplier and Comb Generator}
Designing a Step-Recovery-Diode(SRD) Based on Comb Generator and a
Multiplier circuits are reactively terminated at output port with a higher-order harmonics. thus,  power is partially reflected and recombined to produce stronger harmonics. The damping factor (I) of the SRD is one of the primary drivers in frequency-multiplier or comb-generator design. It is defined as follows:

Ï = (1/2R)(L/C )1/2

where L is the diode’s inductance, C is the diode’s reverse capacitance, and R is the load resistance.

The damping factor (Ï) is between 0.4 and 0.5. If damping is too low, stability problems can arise. If it is too high, the output pulse will become too long.
